Image Clustering Conditioned on Text Criteria

Classical clustering methods do not provide users with direct control of the clustering results, and the clustering results may not be consistent with the relevant criterion that a user has in mind. In this work, we present a new methodology for performing image clustering based on user-specified text criteria by leveraging modern vision-language models and large language models. We call our method Image Clustering Conditioned on Text Criteria (IC|TC), and it represents a different paradigm of image clustering. IC|TC requires a minimal and practical degree of human intervention and grants the user significant control over the clustering results in return. Our experiments show that IC|TC can effectively cluster images with various criteria, such as human action, physical location, or the person's mood, while significantly outperforming baselines.

==> resources/tab_fairness.tex <==
\begin{table}[h!]
\centering\small
\resizebox{\linewidth}{!}
{
\begin{tabular}{l cccc cccc}
\toprule
& \multicolumn{4}{c}{Male ratio} & \multicolumn{4}{c}{Per-group Accuracy}  \\
\cmidrule(lr){2-5} \cmidrule(lr){6-9} 
& Craftsman     & Dancer    & Gardener  & Laborer & Craftsman     & Dancer    & Gardener  & Laborer \\
\midrule
Base Prompt
& 36.4 & 48.6 & 55.3 & 55.8 & 50.0/100.0 & 90.0/95.0 & 100.0/95.0 & 70.0/95.0\\
Fair Prompt
& 44.2 & 50.0 & 55.6 & 50.0 & 80.0/100.0 & 95.0/100.0 & 95.0/95.0 & 60.0/80.0 \\
\bottomrule
\end{tabular}
}
\caption{Male ratio and Per-group accuracy}
\end{table}

% \begin{table}[h!]
% \centering\small
% \begin{tabular}{lcccc}
% \toprule
%  & ACC & NMI & Balance & Entropy \\
% \midrule
% Default     & 86.9  & 0.720 & 36.4  & 1.366 \\
% Fair prompt & 88.1  & 0.722 & 44.2  & 1.375 \\
% \bottomrule
% \end{tabular}
% \caption{1}
% \end{table}


==> resources/tab_hierarchy.tex <==
\begin{table}[t]
\centering\small
\resizebox{\linewidth}{!}{% 
\begin{tabular}{c ccc ccc ccc ccc}
\toprule
\multirow{2}{*}[-3pt]{Method} & \multicolumn{3}{c}{PPMI-7} & \multicolumn{3}{c}{PPMI-2} & \multicolumn{3}{c}{Stanford 10 Location} & \multicolumn{3}{c}{Stanford 2 Location}  \\
\cmidrule(lr){2-4}\cmidrule(lr){5-7}\cmidrule(lr){8-10}\cmidrule(lr){11-13}
& ACC $\uparrow$ & NMI $\uparrow$ & ARI $\uparrow$ & ACC $\uparrow$ & NMI $\uparrow$ & ARI $\uparrow$ & ACC $\uparrow$ & NMI $\uparrow$ & ARI $\uparrow$ & ACC $\uparrow$ & NMI $\uparrow$ & ARI $\uparrow$\\
\midrule
SCAN & 0.632 & 0.540 & 0.442 & 0.850 & 0.505 & 0.489 & - & - & - & - & - & - \\
Ours & 0.964 & 0.928 & 0.921 & 0.977 & 0.842 & 0.911 & - & - & -& - & - & - \\
\bottomrule
\end{tabular}
}
\caption{Control the granularity through text criterion}
\end{table}

==> resources/tab_llmablation.tex <==
\begin{table}[h!]
\centering\small
\begin{tabular}{ccc ccc ccc ccc}
\toprule
\multicolumn{2}{c}{Step 2} & Step 3 &  \multicolumn{3}{c}{CIFAR 10} & \multicolumn{3}{c}{STL 10} & \multicolumn{3}{c}{CIFAR 100} \\
\cmidrule(lr){1-2}\cmidrule(lr){3}\cmidrule(lr){4-6}\cmidrule(lr){7-9}\cmidrule(lr){10-12}
a & b & c & ACC $\uparrow$ & NMI $\uparrow$ & ARI $\uparrow$ & ACC $\uparrow$ & NMI $\uparrow$ & ARI $\uparrow$ & ACC $\uparrow$ & NMI $\uparrow$ & ARI $\uparrow$ \\
\midrule
GPT & GPT & GPT & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\ 
\bottomrule
\end{tabular}
\caption{Male ratio and Per-group accuracy}
\end{table}

% \begin{table}[h!]
% \resizebox{\linewidth}{!}
% {
% \begin{tabular}{|c c c|c c c|c c c|c c c|}
% \hline
% \multicolumn{2}{|c|}{Step 2} & Step 3 &  \multicolumn{3}{c|}{CIFAR 10} & \multicolumn{3}{c|}{STL 10} & \multicolumn{3}{c|}{CIFAR 100} \\
% \hline
% a & b & c & ACC $\uparrow$ & NMI $\uparrow$ & ARI $\uparrow$ & ACC $\uparrow$ & NMI $\uparrow$ & ARI $\uparrow$ & ACC $\uparrow$ & NMI $\uparrow$ & ARI $\uparrow$ \\
% \hline
% a & b & c & 0.617 & - & - & 0.610 & - & - & 0.257 & - & - \\
% \hline
% \end{tabular}
% }
% \caption{Clustering based on object.}
% \end{table}


==> resources/tab_prompt_remove_criteria.tex <==

\begin{table}[h!]
\setlength{\abovecaptionskip}{1pt}
\centering\small
\caption{Text prompts for removing criterion from step2 and step3 during 40-class \texttt{Action}-based clustering on the Stanford 40 Action dataset.}
\resizebox{\linewidth}{!}{
\begin{tabular}{l p{0.9\linewidth}}
    \toprule
    Steps & Prompt \\
    \midrule
    Step 1 & Using the same text prompt as described in Table~\ref{appendix:prompt_action}. \\
    \cmidrule{1-2}
    Step 2a & 
    \texttt{You will be given a description of an image. Your job is to determine the most appropriate label of the image based on the provided description. Please respond in the following format: "Answer: {label}". } \\
    \cmidrule{1-2}
    
        Step 2b & \texttt{You will be provided a list of [\_\_LEN\_\_] image labels and the number of occurrences in a given dataset. Your job is to cluster [\_\_LEN\_\_] words into [\_\_NUM\_CLASSES\_CLUSTER\_\_] labels. Provide your answer as a list of [\_\_NUM\_CLASSES\_CLUSTER\_\_] words, each word representing a label.}\newline\newline

    \texttt{For example, if the input is given as "\{'a': 15, 'b': 25, 'c': 17\}", it means that the label 'a', 'b', and 'c' appeared 15, 25, 17 times in the data, respectively.} \newline\newline

    \texttt{Now you will be given a list of labels and the number of classes, and the list of classes you answered previously.}\newline\newline

    \texttt{Please output a list of clustered labels of length [\_\_NUM\_CLASSES\_CLUSTER\_\_], in the following format: "\{index\}: \{label\}". Make sure that you strictly follow the length condition, which means that {index} must range from 1 to [\_\_NUM\_CLASSES\_CLUSTER\_\_].}\\
    
    \cmidrule{1-2}
    
    Step 3 & \texttt{Your job is to classify the main label of an image. Based on the image description, determine the most appropriate image label that best classifies the image. You must choose from the following options: [\_\_CLASSES\_\_].} \newline\newline \texttt{Give your answer in the following format: "Answer: \{Label\}". Be as specific as possible to choose the closest action from the given list. If a situation arises where nothing is allocated, please assign it to the action that has the closest resemblance.} \\
    % \midrule
    \bottomrule
\end{tabular}
}
\label{appendix_prompt_remove_criteria}
\end{table}

% \renewcommand{\arraystretch}{1}
